Continuum limit of the leading order HQET form factor in $B_s \to K\ell\nu$ decays

We discuss the computation of form factors for semi-leptonic decays of $\rm B$-, $\rm B_s$- mesons in lattice QCD. Considering in particular the example of the static $\rm B_s$ form factors we demonstrate that after non-perturbative renormalization the continuum limit can be taken with confidence. The resulting precision is of interest for extractions of $V_{\rm ub}$. The size of the corrections of order $1/m_{\rm b}$ is just estimated at present but it is expected that their inclusion does not pose significant difficulties.

==> latt_bckp.tex <==
\begin{table}
\begin{center}
\begin{tabular}{cccccccc}
id & $\beta$ & $L/a$ & $a$ [fm] &  $m_\pi$ [{\rm MeV}] & $N_{\rm cfg}$ & $\kappa_s$ & $\theta/(2\pi)$ \\ 
\hline
A5  & $5.2$  &  $32$ &  $0.0749(8)$  &$330$ & $1000$ & $0.13535$  &  $0.034$
\\
F6  & $5.3$ &  $48$ & $0.0652(6)$  &$310$  & $300$ & $0.13579$  &  $0.350$
\\
N6  & $5.5$ & $48$ &  $0.0483(4)$  &$340$  & $300$& $0.13631$  & $0$
\end{tabular}
\caption{Overview of the subset of $N_{\rm f} = 2 $ CLS ensembles on which we performed our measurements.  
Lattice spacings are taken from \cite{Lottini:2014zha}, an update of
\cite{Fritzsch:2012wq}.  All ensembles have $T=2L$ and 
$m_\pi L \geq 4$ where $m_\pi$ is the pion mass. $N_{\rm cfg}$ denotes the number of configurations on which we performed measurements.  The 
hopping parameter of the strange quark is denoted by $\kappa_s$.
The angle $\theta$ appears in the flavour-twisted boundary conditions as explained in the text.} \label{tab:ens}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Lattice Calculation}
\label{s:latt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Framework and Renormalisation}
\label{s:ren}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For our first numerical investigation of the problem, we choose $\nf=2$ 
flavors of quarks. The prime reason for this choice is that in
a related project, the non-perturbative matching of HQET to QCD 
for the currents $V_0,V_k$ is being carried out at the order
$1/\mbeauty$ \cite{DellaMorte:2013ega,Hesse:2012hb,Korcyl:2013ara,Korcyl:2013ega}. 
Once this is complete, we will be able to include
the $1/\mbeauty$ corrections with little additional effort. 
For now, 
we remain at the lowest order of HQET, namely the static order.

The b-quark is then replaced by a static quark \cite{Eichten:1989zv}
labelled ``h''. Two different discretisations, HYP1 and HYP2
are chosen. These have moderate discretisation errors and
a much improved signal-to-noise ratio \cite{DellaMorte:2005yc} compared to the classic Eichten-Hill static
quark action\cite{Eichten:1989zv}. 
The bare currents 
\begin{subequations}
\begin{align}
 V_0^\textnormal{stat} &=  \overline \psi_\textnormal u \gamma_0          \psi_\textnormal h + ac_{\textnormal V_0}(g_0)
 \overline \psi _\textnormal l \sum_l \overleftarrow\nabla^\textnormal S_l \gamma_l          \psi_\textnormal h, \\
V_k^\textnormal{stat} &=  \overline \psi_\textnormal u \gamma_k          \psi_\textnormal h - ac_{\textnormal V_k}(g_0) 
\overline \psi _\textnormal l \sum_l \overleftarrow\nabla^\textnormal S_l \gamma_l \gamma_k \psi_\textnormal h,
\end{align}
\label{deltav}
\end{subequations}
are form-identical to the ones in QCD, apart from the
$\rmO(a)$ improvement terms %\anote{neglecting b-terms!}{}
($\overleftarrow\nabla^\textnormal S$ denotes the symmetric covariant derivative acting on the field to the left).
The coefficients\footnote{Spin symmetry leads to the identity $c_{\textnormal V_k} = c_{\textnormal A_0}$. 
Ref. \cite{Grimbach:2008uy} uses the notation $c_{\textnormal A}^\mathrm{stat},\;c_{\textnormal V}^\mathrm{stat}$ for
$c_{\textnormal A_0},\;c_{\textnormal V_0}$.}, 
$c_{\textnormal V_0}$, $c_{\textnormal V_k}$, are known
to 1-loop order: $c_x=c_x^{(1)} g_0^2 + \rmO(g_0^4)$ with \cite{Grimbach:2008uy}
\begin{subequations}
\begin{align}
 \text{HYP1: }\; c_{\textnormal V_k}^{(1)} = 0.0029(2) \,,\quad
                 c_{\textnormal V_0}^{(1)} = 0.0223(6) \ \\
 \text{HYP2: }\; c_{\textnormal V_k}^{(1)} = 0.0518(2) \,,\quad
                 c_{\textnormal V_0}^{(1)} = 0.0380(6) \,. 
\end{align}
\label{deltav}
\end{subequations}
The multiplicative renormalisation of the bare matrix elements
in \eq{phirgi} follows from the one of the currents,
\begin{align}
 V_0^\mathrm{\RGI} &= Z_\mathrm{A,RGI}^\mathrm{stat} (g_0) 
   Z_\mathrm{V/A}^\mathrm{stat} (g_0) V_0^\mathrm{stat}, 
   \label{v0renorm} \\
 V_k^\mathrm{\RGI} &=  Z_\mathrm{A,RGI}^\mathrm{stat} (g_0)  
   V_k^\mathrm{stat}\,, 
   \label{vkrenorm}
\end{align}
where the notation emphasises that 
$V_k^\mathrm{stat}$ renormalizes exactly as $A_0^\mathrm{stat}$ due to the spin symmetry
of HQET, while for $V_0$ an extra
factor $Z_\mathrm{V/A}^\mathrm{stat} (g_0)$  originates from
the broken chiral symmetry of Wilson fermions.
We use the non-perturbative results 
\bes
  Z_\mathrm{A,RGI}^\mathrm{stat} (g_0) = R(\mu)\, 
  Z_\mathrm{A}^\mathrm{stat}(g_0,a\mu)
\ees
with \cite{DellaMorte:2006sv}
\bes
   R(\mu_0) = 0.880(7) \label{e:RGIfactor}
\ees
relating $A_0^\stat$ at scale $\mu_0=1/L_\mathrm{max}$ in the \SF scheme to the RGI operator and $Z_\mathrm{A}^\mathrm{stat}(g_0,a \mu_0)$, the renormalisation factor at the same scale $\mu$\cite{DellaMorte:2006sv}. The factor $R$ is known 
non-perturbatively by running to very high $\mu$ and continuum extrapolation.
The remaining piece $Z_\mathrm{A}^\mathrm{stat}(g_0,a\mu)$ is reproduced from
 \cite{DellaMorte:2006sv} in \tab{t:zastat}.
For the finite renormalisation $Z_\mathrm{V/A}^\mathrm{stat}$
we use a range
\bes
  [Z_\mathrm{V/A}^\mathrm{stat} (g_0)]^{-1} = 0.97(3)\,.
  \label{e:zva}
\ees
This range is generous, because $Z_\mathrm{V/A}^\mathrm{stat}$ has been seen to be very close to one 
in the quenched approximation \cite{Palombi:2007dt}, and at 1-loop order, there is no $\nf$--dependence. 
Despite these arguments our range in \eqref{e:zva} 
is no more than an educated guess. 
This is adequate since $Z_\mathrm{V/A}^\mathrm{stat}$ affects only one of the $1/\mbeauty$ suppressed terms, which we just use as an illustration of the 
associated uncertainty. Again, we note that such issues %uncertainties 
will be eliminated when the non-perturbative matching is carried out.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\begin{center}
\begin{tabular}{c|cc|cc}
        & \multicolumn{2}{c}{$c_x=0$} & \multicolumn{2}{c}{$c_x=c_x^{(1)} g_0^2$} \\
$\beta$ &  HYP1  &  HYP2  & HYP1  &  HYP2 \\ \hline
$5.2$   & $0.7104(\hphantom{2}5)$ & $0.7920(\hphantom{2}5)$ & $0.7007(\hphantom{2}5)$ & $0.7432(\hphantom{2}5)$ \\
$5.3$   & $0.7057(27)$            & $0.7839(26)$            & $0.6965(27)$            & $0.7376(25)$ \\
$5.5$   & $0.6901(27)$            & $0.7597(26)$            & $0.6820(26)$            & $0.7218(24)$
\end{tabular}
\caption{Values for $Z_\mathrm{A}^\mathrm{stat}(g_0,a\mu) \times 0.8800$. At
$\beta=5.2$ they are taken directly from table 4 of reference \cite{DellaMorte:2006sv}, at $\beta=5.3$ they are obtained using the interpolating polynomial of equation (B.3) and table 9 of that reference and for the $\beta=5.5$ 
numbers we performed a linear extrapolation of the ones at $\beta=5.29$ and $\beta=5.4$.} \label{t:zastat}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Simulation Parameters}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We base our investigation on a subset of the lattice gauge field configurations with
two degenerate flavors of improved Wilson fermions and Wilson gauge action generated by the Coordinated Lattice Simulations (CLS) effort
\cite{Fritzsch:2012wq}. 
The observables are computed on three ensembles, 
namely A5, F6 and N6, chosen to have roughly the same pion mass
but three different lattice spacings, see
\tab{tab:ens}. 
% This allows us to extrapolate the form factor results to the continuum limit. 
The quoted lattice spacings were determined 
from the Kaon decay constant $f_\K$ in reference \cite{Fritzsch:2012wq} and updated in reference \cite{Lottini:2014zha}.

Our choice of the gauge field ensembles fixes the 
degenerate up and down quark masses, $\mlight$. For the spectator strange (valence) quark mass we are free, however, to choose any
smooth function $\mstrange(\mlight)$ which passes through
the physical point. As in \cite{Fritzsch:2012wq} we define this 
function by fixing the
Kaon mass in units of the Kaon decay constant to its physical value
at our (and any) value of $\mlight$. We expect that this will
lead to a flat extrapolation to the physical value of $\mlight$, the ``physical point''.


We choose  $|\vecp_\K|=0.535\,\GeV$ which
corresponds to the minimum available momentum 
with periodic boundary conditions for all fields on the N6 lattice.  
On the other lattices we keep $\vecp_\K = (1,0,0)\,(2\pi +\theta)/L $ 
fixed by introducing flavor-twisted boundary conditions \cite{Bedaque:2004kc} 
$\psi_\mathrm{s}(x+L\hat{1}) = \rme^{i\theta}\psi_\mathrm{s}(x)$,
for the strange quark.  
The $\Bs$-meson is kept at rest by 
$\psi_\mathrm{h}(x+L\hat{1}) = \rme^{i\theta}\psi_\mathrm{h}(x)$,
and we remain with periodic boundary conditions for all other fields.
The numerical values for $\theta$ are listed in \tab{tab:ens}.
Our choice of $\vecp_\K$ yields a central value
of $q^2=21.22\,\GeV^2$ at all lattice spacings and an
error coming from the lattice spacing of $0.03 - 0.05$ $\GeV^2$. 
Note that the flavor-twist is introduced only for  
quenched quarks.
 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Correlation Functions and Matrix Elements}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We work with all-to-all light quark propagators 
\cite{Sommer:1994gg,Foster:1998vw}
implemented by a random U(1) source placed on each time slice 
(``full time dilution''\cite{Foley:2005ac}). 
While this is numerically costly, it significantly reduces the large-time variance. 
Together with the deflated solver 
\cite{ddhmc:webpage,Luscher:2007se,Frommer:2013fsa} that we use, it is thus very 
cost effective. Most notably, this feature of our computation 
provides access to all time separations of two-point and 
three-point functions on our lattices. For details we refer to
\cite{semilept:preparation}.

The two-point functions are defined as
\begin{align}
 \mathcal C^\K (y_0-x_0) & =  \sum\limits_{\vecy, \vecx} \e^{-\im \vec p \cdot (\vecy - \vecx)} \langle P_{\textnormal{s} \textnormal{u}} (y)P_{\textnormal{u} \textnormal{s}}(x)  \rangle ,  \label{ck} \\
  \mathcal C^\B_{ij} (y_0-x_0)  &=  \sum\limits_{\vecy, \vecx} \langle P^{(i)}_{\textnormal{s}\textnormal{b}}(y)P^{(j)}_{\textnormal{b}\textnormal{s}}(x)  \rangle , \label{cb} 
\end{align}
with the pseudoscalar density $P^{(i)}_{\textnormal{q}_1 \textnormal{q}_2} (x) = \overline{\psi}_{\textnormal{q}_1} (x) \gamma_5 \psi_{\textnormal{q}_2} (x) $. 
Indices $i$ and $j$ denote the use of different Gaussian wave functions for the light quarks
with a set of smearing parameters as in \cite{Bernardoni:2013xba}.
Up to terms which are exponentially suppressed in the time extent 
$T$ of the torus, we can 
parameterise $\mathcal C ^\K , \mathcal C^\B $ as
\begin{align}
 \mathcal C^\K (t_\K) &\simas{t_\K \gg a} \sum_n \big(\kappa^{(n)}\big)^2   \e^{-E_\K^{(n)} t_\K} \approx \big(\kappa^{(0)}\big)^2 \e^{-E^{(0)}_\K t_\K}, \label{e:ckek} \\
 \mathcal C^\B_{ij} (t_\B) &\simas{t_\B \gg a} \sum_n \beta_i^{(n)}  \beta_j^{(n)} \e^{-E_\B^{(n)} t_\B} \approx \sum\limits_{n=0}^N \beta_i^{(n)}  \beta_j^{(n)} \e^{-E_\B^{(n)} t_\B} ,  \label{e:cbeb} 
\end{align}
where we have denoted amplitudes by 
$\kappa^{(n)}=L^{3/2} (2E_\K)^{-1/2}\langle 0 | P_{\textnormal{u}\textnormal{s}}(0) |K,n\rangle$ and
$\beta^{(n)}_i=L^{3/2} (2E_\B)^{-1/2}\langle 0 | P^{(i)}_{\textnormal{s}\textnormal{b}}(0) |K,n\rangle$, while energies are labeled $E_\K^{(n)}, E_\B^{(n)}$.  The restrictions $t_x\gg a$ are required 
because we use an improved action where the positivity of the 
transfer matrix is not guaranteed. 
In a fit to these correlation functions, we use $t$-ranges denoted by $\tfit{K2}{min} \le t_\K \le \tfit{K2}{max}$
and $\tfit{B2}{min} \le t_\B \le \tfit{B2}{max}$, respectively, and
$N$ is the number of excited $\B$-meson states which we include.
Note that we have restricted ourselves here to only the ground state of the Kaon. %, which we find to be a good approximation.
There is a single, fixed, 
smearing level for the Kaon. In the Kaon two-point function,
ground state dominance sets in at around 1.2~fm, while for the \B\-meson 
this happens a bit earlier for our optimal (widest) Gaussian wave function. An illustration is found in \Fig{plat} which also shows that a good precision is reached which appears to be 
significantly better than in previous computations of B- or \B-meson 
form factor computations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{center}
\begin{figure}
%\hspace{-.5cm}\scalebox{0.3}{\includegraphics{plots/p14.pdf} }
\scalebox{0.6}{\includegraphics{plots/effM_EK.pdf} }
\scalebox{0.6}{\includegraphics{plots/effM_EBs_hyp2.pdf} }

\caption{Effective energy of $\cC_\K$ (left)
and $\cC_\B$ (right) on ensemble N6.  There are decent plateaus 
with small errors even though the kaon carries a non-vanishing momentum and we have a static $\B$-meson.  The value for the ground state energies as obtained from the fit is shown as a red band. Uncertainties shown here are only those of $E^\textnormal{stat}$ and $E_\K$ in lattice units, not the ones of $\mhbare$ and
the lattice spacing. The data points are shown for the case of maximum smearing,
while the fit involves all the smearing levels.
}
\label{f:plat}
\end{figure}
\end{center}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



The three-point function % ($t_\K=,\,t_\B=x^0_v-x^0_i$)
\begin{equation}
 \mathcal C^{\B\to\K}_{\mu,j} (x^0_f-x^0_v, x^0_v-x^0_i) = \sum\limits_{\vecx_f, \vecx_v, \vecx_i} \e^{-\im \vecp \cdot (\vecx_f - \vecx _v)} \langle P_{\textnormal{d}\textnormal{u}}(x_f) V^\mu(x_v) P_{\textnormal{b}\textnormal{d}}^{(j)} (x_i) \rangle \label{c3}.
\end{equation}
has a representation
\begin{align}
  \Ct_{\mu, i}(t_\K,t_\B) &\simas{t_\K,t_\B \gg a}  \sum\limits_m  \sum\limits_n \kappa^{(m)}  \varphi_\mu^{(m,n)} \beta_i^{(n)} \e^{-E^{(m)}_\K t_\K}  \e^{-E^{(n)}_\B t_\B}  \nonumber \\ 
& \approx \sum\limits_{n=0}^N \kappa^{(0)}  \varphi_\mu^{(0,n)} \beta_i^{(n)}   \e^{-E^{(0)}_\K t_\K} \e^{-E^{(n)}_\B t_\B}\,.
  \label{e:c3eb}
\end{align}
In our fits to $\Ct_{\mu, i}$ we consider $(t_\K,t_\B)$-values restricted to the rectangle with
$\tfit{K3}{min} \le t_\K \le \tfit{K3}{max,\mu }$ and $\tfit{B3}{min} \le t_\B \le \tfit{B3}{max,\mu}$.

The desired form factors are given by the ground state matrix elements 
\begin{subequations}
\begin{align}
\fparallel^\hqetb  &=  \varphi^{(0,0)}_0 \sqrt{2E_\K}\, , \label{fparphi}  
\\
\fperp^\hqetb      &=  \frac{\varphi^{(0,0)}_k}{p_\K^k}\, \sqrt{2E_\K}\,.\label{fperphi}
\end{align}
\label{symffphi}
\end{subequations}
Their extraction from the data is rather delicate because 
statistical errors grow with time separations. Due to our 
all-to-all computation and the use of HYP1, HYP2 discretisations, 
we still have a precision of better than two percent for 
$t_\K$ and $t_\B$ around \anote{fix}{1.x fm}, in particular the 
precision of the three-point 
function reaches the two percent level around $t_\K + t_\B =$  \anote{add}{2.x fm}.
However, in this range we find that $N=2$ excited states are necessary 
to obtain a good description of the data and a safe extraction
in particular of the most important form factor $\varphi^{(0,0)}_k$. 
Details will be described in \cite{semilept:preparation}.

To determine the reliability of the fits, we vary the boundaries
$\tfit{B2}{min}$, $\tfit{K3}{min}$, and $\tfit{B3}{min}$
of the fit ranges (the other boundaries are determined by \anote{mention noise and wrappers? RS: yes}{xxx})
and verify that the fit results remain unchanged within errors.
As an example, fig. xxx shows the dependence of the fit result for 
$\varphi^{(0,0)}_0$ and $\varphi^{(0,0)}_k$ on $\tfit{K3}{min}$ 
and $\tfit{B3}{min}$.
\\[3ex]
{\cred discuss scatter plots when available}
\\[3ex]
The bare ground state matrix elements are listed in \tab{t:bareff}.

\begin{center}
\begin{figure}
%\hspace{-.5cm}\scalebox{0.3}{\includegraphics{plots/p14.pdf} }
\scalebox{0.3}{\includegraphics[angle=270]{plots/phi0.pdf} }
\scalebox{0.3}{\includegraphics[angle=270]{plots/phi1.pdf} }

\caption{Scatter plots for the bare form factors $\varphi^{(0,0)}_0$
  (left) and $\varphi^{(0,0)}_1$ (right) as a function of
  $t^{B3}_{min}$ (different groups) and $t^{K3}_{min}$ (inside the
  groups). $t^{B3}_{min}-t^{B2}_{min}$ is kept fixed.  }
\label{f:scatter}
\end{figure}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[p!]
\begin{center}
\begin{tabular}{llllll}
 \multicolumn{2}{c}{discretisations:}    &   \multicolumn{2}{c}{$c_x=0$} &   
                    \multicolumn{2}{c}{$c_x=c_x^{(1)}g_0^2$} \\
     &  $\beta$          & HYP1 &  HYP2  & HYP1 &  HYP2  \\
\hline
\input{tables/bareff.tex}
\\
\end{tabular}
\caption{The unrenormalized form factors $\fparallel,\fperp$ for the specified 
discretisations.}
\label{t:bareff}
\end{center}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[p!]
\begin{center}
\begin{tabular}{lcccccccccc}
$\beta$ & $\tfit{K2}{min}$ & $\tfit{K2}{max}$ & $\tfit{B2}{min}$ & $\tfit{B2}{max}$  
& $\tfit{K3}{min}$ & $\tfit{K3}{max,0}$ & $\tfit{K3}{max,1}$ & $\tfit{B3}{min}$ & $\tfit{B3}{max,0}$ & $\tfit{B3}{max,1}$ 
\\
\hline
\input{tables/fitrange.tex}
\\
\end{tabular}
\caption{Ranges of $t_\K$ and $t_\B$ used in our final fit
leading to \tab{t:bareff}.}
\label{t:fitrange}
\end{center}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Continuum Limits}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[p!]
\begin{center}
\begin{tabular}{llllll}
 \multicolumn{2}{c}{discretisations:}    &   \multicolumn{2}{c}{$c_x=0$} &   
                    \multicolumn{2}{c}{$c_x=c_x^{(1)}g_0^2$} \\
     &  $\beta$          & HYP1 &  HYP2  & HYP1 &  HYP2  \\
\hline
\input{tables/rgiff.tex}
\\
\end{tabular}
\caption{Renormalized form factors $\fparallel^\RGI,\fperp^\RGI$ and their
continuum limits. The last line gives the conventional combination of
form factors, 
$f_+$.}
\label{t:rgiff}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The bare form factors, renormalized as explained in \sect{ren}, yield the RGI form factors listed in \tab{t:rgiff}. Their errors take account of 
all statistical correlations and autocorrelations as described in 
\cite{Bernardoni:2013xba} based on
\cite{Wolff:2003sm,Schaefer:2010hu}. Irrespective of the discretisation,
they show a weak dependence on the lattice spacing, which we illustrate
in \fig{contlim}. Therefore it is no obstacle that we know the 
O$(a)$ improvement coefficients of the currents only in 1-loop perturbation theory. These coefficients are not very relevant at the level of precision of our data.\footnote{The reader
should not be confused by the fact that bare numbers may depend significantly
on $c_x$; discretisation errors have to be assessed after renormalisation.
}

As our best result we estimate the continuum limit by a linear extrapolation in $a^2$ of the data with $c_x=c_x^{(1)}g_0^2$, as illustrated in the figure. For $\fparallel$ a simple constant extrapolation (a weighted average)
yields compatible results, but of course with much smaller error bars. Since there is no reason, why $a^2$ effects should be entirely absent,
we use the numbers with the larger error bars. 

Finally we combine the continuum limits of HYP1 and HYP2 in a weighted 
average,
\begin{subequations}
\begin{align}
\fparallel^\RGI  &= \hsnew{ xxx \GeV^{1/2} }, \label{e:resfpar}  
\\
\fperp^\RGI      &= \hsnew{ xxx \GeV^{-1/2} }\,.\label{e:resfperp}
\end{align}
\label{e:resfrgi}
\end{subequations}

\subsection{The Form Factors $f_+$ and $f_0$, and Comparison to Other Results}

%%% \subsubsection{The form factor $f_+$}
We now have different options to estimate the form factor $f_+$. 
Working only at static order, we can use
any quantity $\fplusnum{i}$ with
\bes
  f_+  = \fplusnum{i} \cdot \left[ 1 + \rmO(1/\mbeauty) \right] \;, %%% ; i=1,2% 
\ees
and we consider (dropping the argument of $C_\mathrm{V_0},C_\mathrm{V_k}$)
\begin{subequations}
\begin{align}
\fplusnum{1}  &= \sqrt{m_\B/2}\,\left( (1-\frac{E_\K}{m_\B}) \,C_\mathrm{V_k}\,\fperp^\RGI(E_\K) +
  \frac{1}{m_\B}\,C_\mathrm{V_0}\,\fparallel^\RGI(E_\K)\right)\,,
\label{e:fplus1}  
\\
\fplusnum{2}    &= \sqrt{m_\B/2} \,C_\mathrm{V_k}\,\fperp^\RGI(E_\K) 
\,,\label{e:fplus2}
%\\
%\fplusnum{3}        &= \,.\label{e:fplus3}
\end{align}
\label{e:resfplus}
\end{subequations}
In $\fplusnum{1}$ all known terms and kinematical factors are taken into 
account, despite the 
fact that the form factors $\fparallel$ and $\fperp$ contain further $1/\mbeauty$ suppressed contributions 
which we do not control, while in $\fplusnum{2}$ we systematically 
drop all $1/\mbeauty$ suppressed contributions.  Numerically we have
(combined HYP1/2)
\begin{subequations}
\begin{align}
\fplusnum{1}  &= 1.77(7)\,,
\label{e:fplus1num}  
\\
\fplusnum{2}        &= 1.63(8)
\,.\label{e:fplus2num}
%\\
%\fplusnum{3}        &= \,.\label{e:fplus3}
\end{align}
\label{e:resfplus}
\end{subequations}
Of course one could also include in \eqref{e:fplus2} the exactly 
known kinematical pre-factor of $\fperp$ via
$\fplusnum{3} = (1-{E_\K}/{m_\B})\,\fplusnum{2} = 0.864\times\fplusnum{2}$.
Such \anote{reall 15\%}{$\sim 15\%$} uncertainties/ambiguities will be reduced to $1\% - 2\%$ 
when we include all $1/\mbeauty$ terms.

In order to give a single number, we estimate the O$(1/\mbeauty)$ terms in this way
and quote 
\bes
  f_+(21.22 \GeV^2) = \fplusnum{2} \pm 0.15 \, \fplusnum{2} = 1.63(8)\pm 0.24\,.
  \label{e:fplusfin}
\ees

%%% \subsubsection{The Form Factor $f_0$}
Besides $f_+$ it is common in the literature to report results for 
the scalar form factor $f_0$, which is another linear combination
of $\fperp$ and $\fparallel$. To estimate its value, we use
\beq
\fzeronum{1}  = \frac{\sqrt{2/m_\B}}{1-m_\K^2/m_\B^2}\, \left( 
  (1-\frac{E_\K}{m_\B}) \,C_\mathrm{V_0}\,\fparallel^\RGI(E_\K) +
  \frac{\vecp_\K^2}{m_\B}\,C_\mathrm{V_k}\,\fperp^\RGI(E_\K)\right)\,,
\label{e:fzero1}  
%%%\\
%%%\fzeronum{2}        &= \sqrt{2}m_\B^{-3/2} \frac1{1-m_\K^2/m_\B^2}\,
%%%           C_\mathrm{V_0}\,\fparallel^\RGI(E_\K)  \,,\label{e:fzero2}
\eeq
where, analogous to $\fplusnum{1}$, all known kinematic O$(1/\mbeauty)$-terms are included.
Our (combined HYP1/2) result is
\beq
\fzeronum{1} = 0.66(3)
\label{e:zero1num}  
\eeq

%%% \subsubsection{Comparison to Other Results}

Our results, \eq{fplusfin} and \eq{zero1num} compare rather well with 
other values of the form factors in the literature. Flynn et al.
\cite{Flynn:2015mha} report a value for $f_+ \approx 1.65 (10) $
and $f_0 \approx 0.62 (5) $, while Bouchard et al. \cite{Bouchard:2014ypa} quote 
$f_+ \approx  1.80 (20) $ and $f_0 \approx 0.66 (5) $ for
values of $q^2$ matching ours well within errors.  
As should be clear our estimates have a systematic error of a completely 
different nature. While the continuum limit is taken very 
accurately we neglect a dependence on the light quark mass 
which -- according to \cite{Flynn:2015mha, Bouchard:2014ypa} -- is below our errors.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!h]
\begin{center}
\hspace{0cm}\scalebox{0.56}{\includegraphics{plots/f_par.pdf} }
\hspace{0cm}\scalebox{0.56}{\includegraphics{plots/f_perp.pdf} }
\caption{Results for $\fparallel^\RGI$ (left) and $\fperp^\RGI$ (right) 
with 1-loop O$(a)$ improvement coefficients. Data for actions HYP1/2 
are separated slightly in $a^2$ for better visibility. 
The lines show continuum extrapolations linear in $a^2$.
}
\label{f:contlim}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

